WALL-SS: Scaling Long-horizon World Models via Next-Scale Autoregression

Generative world models provide robots with predictive models of how the world evolves under interaction, with growing potential for simulation, planning, policy evaluation, and robot learning. Beyond clip-level future prediction, a unified generative formulation should relate actions to consequences, support flexible horizons and continuous interaction, and enable reward-driven optimization. We introduce WALL-SS, a world model that generates visual futures through Scale-wise autoregressive Scaling, enabling action-controllable and long-horizon robotic simulation. WALL-SS represents embodied trajectories as causal sequences of temporally interleaved observations and actions, making action-dependent state transitions explicit while naturally supporting variable-length generation, streaming extension through reusable causal states, and direct optimization through sequence probabilities. To make this formulation effective over long horizons, we generate each future observation in a coarse-to-fine manner and develop three complementary components within the same hierarchy. Action-conditioned next-scale prediction injects scale-aligned action representations to improve action-future coupling and model both successful and failed behaviors. Scale-compressed long-horizon memory retains recent interactions at fine resolution while compressing distant observations and actions, with scale-wise dream forcing enhancing robustness to self-generated context. Finally, on-policy alignment optimizes autoregressive visual dynamics with action-following and long-term consistency rewards while preserving the pretrained visual distribution. Experiments show that WALL-SS improves action following and trajectory accuracy, supports coherent minute-long streaming rollout under bounded memory, and consistently benefits from on-policy alignment in reducing action drift and long-horizon inconsistency.

==> preamble.tex <==
\setlength{\headheight}{17.8264pt}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{neurips_2025}
\usepackage[bookmarks=true]{hyperref}
\usepackage{url}
\usepackage{booktabs}
\usepackage{amsfonts}
\usepackage{nicefrac}
\usepackage{microtype}
\usepackage{xcolor}
\usepackage{fix-cm}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{eso-pic}
\usepackage{xspace}

\usepackage{times}
\usepackage{xspace}

% \usepackage[numbers]{natbib}
% \usepackage{caption}
% \captionsetup[table]{name=Table, labelsep=period, font=footnotesize}
% \captionsetup[figure]{name=Fig., labelsep=period, font=footnotesize}
% \usepackage{multicol}
% \usepackage[nameinlink,noabbrev]{cleveref}

% \usepackage{multirow}
% \usepackage{multicol}
% \usepackage[table]{xcolor}

% customized commands
\newcommand{\mike}[1]{\textit{\textcolor[rgb]{0.00,0.0,0.80}{[mike]~#1~}}}
\newcommand{\ours}{\textsc{WALL-ARWM}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}

% mathematial
